Once Again, with Style: Understanding and Supporting Partial Reuse in Dashboard Authoring

Presentation-oriented tasks including formatting and layout design are critical but often neglected aspects of dashboard authoring given their labor intensive nature. In this work, we follow a user-centered design approach to explore ways that partial reuse of pre-existing dashboards may support the dashboard design process. Based on collective feedback from 10 professional dashboard creators, we contribute: (a) findings from a formative study characterizing dashboard reuse needs and challenges; and (b) reflections and opportunities from a concept validation study with ReDash, a design probe for partial reuse of dashboard presentation features (style and layout) from multiple sources.

==> Sections/2.related_work.tex <==
\vspace{-0.8em}
\section{Related Work}

Several studies discuss the need for richer reuse and example-centered tools for visualization and dashboard authoring. 
Bako et al.~\cite{bako2022understanding} discuss the role of examples in visualization authoring and outline strategies that designers use to leverage these examples; whereas 
 %also highlight a need to streamline dashboard design by allowing content reuse.
Tory et al.~\cite{tory2021finding} and Bach et al.~\cite{bach2022dashboard} both highlight the need for tools for reusing and repurposing content from other dashboards for a more streamlined authoring experience. 
Conversely, several \textit{design-focused} approaches\,---\,i.e., aiding with features such as layout composition and style\,---\, have been explored for dashboard authoring. These include
%These systems can be divided into two categories: content-focused, and design-focused.
%\textit{content-focused systems}, aimed at recommending \emph{what} to show in a dashboard (i.e., charts and widgets)
%~\cite{wu2021multivision,pandey2023medley,srinivasan2023bolt,choi2025waltzboard,srinivasan2023bolt,soni2024survey, deng2022dashbot, epperson2023declarative}.
template generation from reference images and sketches~\cite{ma2020ladv} and natural language prompting~\cite{shen2025dashchat}, plus works that leverage design rules~\cite{lin2023dminer} and domain-specific languages~\cite{jiang2022mod2dash} to model design choices~\cite{lin2023dminer, chen2020composition, shi2022colorcook}, recommend effective layouts~\cite{chen2020composition, zeng2023semi}, and configure new dashboards~\cite{shen2025dashchat,ma2020ladv}.
%For instance, LADV~\cite{ma2020ladv} allows authors to provide an image or rough sketches as examples and suggests dashboard templates with preset charts and layouts for further customization.
%DMiner~\cite{lin2023dminer} leverages layout optimization rules derived from a repository of dashboards to recommend effective layouts given a set of views.
%Mod2Dash~\cite{jiang2022mod2dash} takes a domain-specific language (DSL) approach to allow dashboard designers to model their design choices for a dashboard's layout, chart design (e.g., axes, colors), and interaction between views. The system then leverages this DSL to automatically configure new dashboards with these modeled defaults, promoting design reuse.
To our knowledge, our work is the first to explore and conceptualize the notion of dashboard reuse from prior exemplars within dashboard authoring workflows.
%dashboard reuse design via the \textit{reuse of presentation elements from exemplar dashboards}.
%authors to reuse content to create dashboards based on existing content.

%The concept of style transfer is well aligned with this notion of reuse, and has been broadly explored in the context of web design~\cite{fitzgerald2008copystyler,kumar2011bricolage} and images plus vector graphics~\cite{warner2023interactive, swearngin2018rewire, lu2025misty}, but remains relatively underexplored in the context of dashboard authoring. We draw inspiration from the aforementioned systems in the broader user interface and graphics design and build upon them in the context of dashboard design.

\arjun{high-level suggestion: we can merge sec 1 and 2 into an "Introduction and Background" to have a better flow. I can take a shot at this if there's agreement}

\vspace{-1em}

\begin{comment}

\subsection{Reuse in Data Visualization}

\textbf{Understanding reuse practices.}
Bako et al.~\cite{bako2022understanding} outlined strategies that designers use to leverage data visualization examples. This includes (a)selecting and merging multiple examples, (b) replicate and modify, and (c) trial and error. They also identify challenges to reuse, including (a) significant time spent modifying examples, and (b) the difficulty of translating examples across formats and authoring tools. Also, a desire for "automation to aid, not replace", which emphasizes the idea of minimizing repetitive work while supporting creative expression, and point to an opportunity for easier authoring of visualizations with examples as inputs.

\textbf{Style extraction and transfer for UI and creative designs.}

CopyStyler~\cite{fitzgerald2008copystyler} and  Bricolage~\cite{kumar2011bricolage} support design and layout transfer between web designs.

Bricolage~\cite{kumar2011bricolage} does so via a component matching algorithm that accounts for semantic and structural properties of components.

Rewire~\cite{swearngin2018rewire} extracts vector representations of interface components from example designs provided as images.

Warner et al. proposed VST~\cite{warner2023interactive} which enables style transfer between two vector graphics via a structural graph representation and matching approach.

Misty~\cite{lu2025misty} supports conceptual blending of UI components with code generation.

\textbf{Data and style reuse for visualizations.}

iVolver~\cite{mendez2016ivolver} supports data extraction from bitmap images and subsequent mark manipulation.

ChartSense~\cite{jung2017chartsense} proposes a technique to extract data from chart images.

Harper and Agrawala~\cite{harper2017converting} propose a technique to deconstruct a D3 visualization into a reusable template.

\subsection{Dashboard Styling}

And while commercial dashboarding tools provide features for styling and layout reuse (such as PowerBI report templates\footnote{\url{https://learn.microsoft.com/en-us/power-bi/create-reports/desktop-templates}} and Tableau custom themes~\footnote{\url{https://help.tableau.com/current/pro/desktop/en-us/formatting_custom_themes.htm}}), this modality of reuse only supports a single styling source. 

LADV \cite{ma2020ladv}, which focus on using exemplars to kick-start design, while arguing for the limitations of both templates and bespoke designs. However, they do not support iterative integration of design features from multiple sources. 

 This notion has been extended to a number of visual structured artifacts beyond images, including vector graphics~\cite{}, web and UX design~\cite{}, and single data visualizations~\cite{}, but not multi-view dashboards. 


% intent capturing / intent translation / ...

\subsection{Bridging design intent and design attributes}

Draco~\cite{moritz2018formalizing} proposes a constraint based approach to formally apply visualization design heuristics.

Scout~\cite{swearngin2020scout} leverages user-specified high-level constraints to generate interface design alternatives.

In the context of web design, Stylette~\cite{kim2022stylette} interprets design intent from natural language utterances to surface a list of visual CSS attributes that can be manipulated to fulfill design goals.


\subsection{Dashboard authoring systems}

redash{} proposes a new approach to dashboard design by combining an intent-driven reuse pipeline with a grammar-based representation of dashboards and an LLM-backed interface. Unlike commercial tools such as Tableau and Power BI, which support dashboard creation but lack structured mechanisms for reusing design elements across dashboards, ReDash enables users to extract, match, and apply layout and style attributes from reference dashboards considering different intent levels, by primarily leveraging dashboard images. 

While previous work has explored design automation and recommendation (e.g., DMiner’s layout mining \cite{lin2023dminer}, MultiVision’s deep learning–based layout generation \cite{wu2021multivision}, and Mod2Dash’s model-driven pipeline \cite{jiang2022mod2dash}), these systems primarily automate dashboard creation rather than support design reuse. 

Others like BOLT \cite{srinivasan2023bolt} and DashChat \cite{shen2025dashchat} leverage natural language for authoring but do not explicitly support reuse workflows. Meanwhile, recommender systems such as MEDLEY \cite{pandey2022medley} and VizCommender \cite{oppermann2020vizcommender} help users discover visualizations but do not particularly focus on design dimensions. 

 In contrast to systems like Plume \cite{lisnic2025plume} and Azimuth \cite{srinivasan2023azimuth}, which support specific dashboard authoring needs such as text generation or accessibility, \redash{} supports design extraction and application in an end-to-end reuse workflow.

 \end{comment}


==> Sections/7.conclusion.tex <==
%\section{Conclusion}

% From design requirements derived from a interview- and task-based formative study with professional dashboard creators, we scoped our design and implementation efforts to aspects of dashboard \textit{styling and layout}, which emerged as critical authoring pain points.  Using \redash{} as a design probe, we presented the notion of partial reuse to dashboard authors, which helped us better understand not only its particular application of reuse but also informed other facets of reuse that are worth pursuing. 
